Towards a Computational Analysis of Suspense: Detecting Dangerous Situations

Suspense is an important tool in storytelling to keep readers engaged and wanting to read more. However, it has so far not been studied extensively in Computational Literary Studies. In this paper, we focus on one of the elements authors can use to build up suspense: dangerous situations. We introduce a corpus of texts annotated with dangerous situations, distinguishing between 7 types of danger. Additionally, we annotate parts of the text that describe fear experienced by a character, regardless of the actual presence of danger. We present experiments towards the automatic detection of these situations, finding that unsupervised baseline methods can provide valuable signals for the detection, but more complex methods are necessary for further analysis. Not unexpectedly, the description of danger and fear often relies heavily on the context, both local (e.g., situations where danger is only mentioned, but not actually present) and global (e.g., "storm" being used in a literal sense in an adventure novel, but metaphorically in a romance novel).

==> resources/base.tex <==
\begin{description}
\item[Fear] ängstlich, panisch, entsetzt, entsetzlich, besorgt, Angst, Furcht, Panik, furchtbar, fürchterlich, wehrlos, verzweifeln, verzweifelt, erschrecken, Schreck, Schrecken, erschreckt, erschrocken, schrecklich, verängstigt, panisch, grässlich, schmerzhaft, höllisch, hilflos, scheußlich, hoffnungslos, Bedrohung, bedroht, bedrohlich, nervös, überwältigen, überwältigt, lähmen, lähmend, gelähmt, widerlich, unheimlich, leiden, leiden, leidend, beunruhigt, Beunruhigung, beunruhigen, beunruhigend, Gefahr, gefährlich, gefährdet, gefahrvoll
\item[Abduction] Entführer, Kidnapper, Kidnapping, kidnappen, entführen, Gewalt, gefangen, gefesselt, geknebelt, fesseln, knebeln, eingesperrt, einsperren, entführt, gekidnappt
\item[Fire] Feuersturm, Feuer, Brand, Explosion, brennen, löschen, prasseln, verbrennen, lodern, Verbrennung, explosionsartig, Hausbrand, Gebäudebrand, abfackeln, abgefackelt, niedergebrannt, verbrannt, Brandbeschleuniger, Brandstiftung, Brandstifter, anzünden, angezündet, entzündet, Großbrand
\item[Violence] Messer, zustechen, einstechen, stechen, zuschlagen, einschlagen, schlagen, töten, ermorden, morden, Gewalt, Gewaltverbrechen, schleifen, erschlagen, erstechen, schießen, erschießen, packen, beißen, zubeißen, verbeißen, erwürgen, würgen, erdrosseln, zuschnüren, abschnüren, Dolch
\item[War] Krieg, Gefecht, Kampf, Krieger, Truppe, Truppen, Kommandant, Kriegsschiff, Feind, Soldat, Offizier, Kamerad, Stellung, Posten, Gewehr, Maschinengewehr, Unteroffizier, General, Oberleutnant, Leutnant, Bunker, Graben, Schützengraben, Panzer, Flotte, Kriegsflotte, Heer, Schlachtschiff, Bombe, Flugzeug, Staffel, Flieger, Kampfflugzeug, Kreuzer, Zerstörer
\item[Storm] Unwetter, donnern, Sturm, Wolkenbruch, Gewitter, Orkan, Gewittersturm, regnen, Donner, prasseln, Hagelschauer, Hagelschlag, Schneesturm, hageln, Gewitterregen, Donnerwetter, Sturmwind, Hagelsturm, Schneestürme, Sturmböen, schneien, Schneeregen, Regengüssen, Regenwetter, Regenfall, Regengüsse, Schneefall, Starkregen, Gewitterschauer, Blitz, Regen, Wind, Windstoß, Hagel
\item[Duel] Kampf, Gegner, Duell, Klinge, Schwert, Messer, Pistole, Zweikampf, Feind, Sieger, kämpfen, duellieren, Waffe, Opfer, Wunde, stoßen, rammen, wild, erbittert, aufeinander, einschlagen, schlagen, Streit, Widersacher, Gegenüber
\item[Overall Danger] Gewalt, Kriegsschiff, Gewehr, schlagen, gefangen, Schlachtschiff, einstechen, Schützengraben, knebeln, Hausbrand, Gewitterregen, zuschlagen, erstechen, Truppe, morden, Hagelschlag, Großbrand, kidnappen, Kidnapping, Opfer, zustechen, stoßen, zubeißen, Zerstörer, prasseln, Brandbeschleuniger, Krieg, Gewitter, verbeißen, Gewitterschauer, Bombe, Kommandant, zuschnüren, Staffel, abschnüren, Pistole, Maschinengewehr, Regenwetter, Regengüssen, Explosion, lodern, erschießen, Feuersturm, Panzer, Schneesturm, Dolch, würgen, donnern, Hagelsturm, entführen, Graben, Wolkenbruch, Flieger, angezündet, geknebelt, erschlagen, Regenfall, Oberleutnant, verbrannt, Posten, löschen, Widersacher, Sturm, Zweikampf, packen, anzünden, schießen, Brandstiftung, Klinge, Streit, Hagel, fesseln, schneien, erwürgen, explosionsartig, abgefackelt, rammen, Feind, Soldat, Krieger, Offizier, Heer, Schwert, Schneeregen, Leutnant, hageln, verbrennen, Wind, Kamerad, Kampf, beißen, Kriegsflotte, gefesselt, erdrosseln, Duell, Regen, Unteroffizier, Unwetter, General, entführt, Donner, schleifen, Starkregen, Gegner, eingesperrt, Schneefall, töten, ermorden, Flugzeug, Gebäudebrand, kämpfen, Regengüsse, aufeinander, Sturmböen, Feuer, wild, Bunker, brennen, Donnerwetter, Verbrennung, Truppen, Sturmwind, niedergebrannt, Windstoß, Gegenüber, Gewaltverbrechen, einsperren, Kreuzer, Orkan, entzündet, Entführer, Hagelschauer, Schneestürme, stechen, Waffe, Gefecht, abfackeln, Blitz, gekidnappt, regnen, Wunde, erbittert, einschlagen, Kampfflugzeug, Flotte, Kidnapper, Brand, Messer, Stellung, Brandstifter, Sieger, duellieren, Gewittersturm
\end{description}

==> resources/conceptnet.tex <==
\begin{description}
\item[Fear] ängstlich, panisch, entsetzt, entsetzlich, besorgt, angst, furcht, panik, furchtbar, fürchterlich, wehrlos, verzweifeln, verzweifelt, erschrecken, schreck, schrecken, erschreckt, erschrocken, schrecklich, verängstigt, panisch, grässlich, schmerzhaft, höllisch, hilflos, scheußlich, hoffnungslos, bedrohung, bedroht, bedrohlich, nervös, überwältigen, überwältigt, lähmen, lähmend, gelähmt, widerlich, unheimlich, leiden, leiden, leidend, beunruhigt, beunruhigung, beunruhigen, beunruhigend, gefahr, gefährlich, gefährdet, gefahrvoll, beängstigend, gefährdung, ominös, torschlusspanik, brenzlig, suchtkrank, ohne, einsturzgefahr, diabolisch, ohnmächtig, mächtig, verstörung, demokratiegefährdend, schmerzend, schreckenerregend, vogelfrei, kommend, kränkeln, naturschutz, gefahrbringend, risikoreich, muskel, unbeweglich, suspekt, lebensbedrohlich, degoutant, querschnittsgelähmt, rechtlos, leidensdruck, unbeholfen, kolossal, verdattert, lahm, brüchig, ausserordentlich, fassungslos, ungeheuer, ratlos, schock, aussichtslos, höhenangst, gärung, dämonenspiel, aufgeregt, garstig, verbunden, bevorstehend, toll, raketenwarnung, dolent, deprimierend, drangsal, schutzlos, h, schmerzvoll, schändlich, belastend, unbeschützt, trunken, frostbeule, äthern, bedrohen, feige, not, verwundbar, gruselig, beängstigen, leid, paralysieren, panikartig, gefahrenreich, infernalisch, ernüchternd, sorge, wehren, überstehen, scheusslich, religion, schaurig, kampf, ruhig, kopfscheu, verzagen, umwerfen, angsteinflössend, komplex, bangen, recht, betroffen, medizin, krampfhaft, lähmung, gräuel, bezweifeln, entsetzen, abenteuer, befangen, bedrücken, nicht, bang, bewegungsunfähig, ausweglos, tückisch, entrinnen, unwohl, gel, hart, kafkaesk
\item[Abduction] entführer, kidnapper, kidnapping, kidnappen, entführen, gewalt, gefangen, gefesselt, geknebelt, fesseln, knebeln, eingesperrt, einsperren, entführt, gekidnappt, gef, inhaftieren, gefangener, geiselnahme, schanghaien, umgangssprachlich, freiheit, kindesentführer, frei, geiselnehmer, mitgefangener, gefängnis, luftpirat, erpressen, entführung, festsetzen, käfig, gefangenschaft, flugzeugentführer
\item[Fire] feuersturm, feuer, brand, explosion, brennen, löschen, prasseln, verbrennen, lodern, verbrennung, explosionsartig, hausbrand, gebäudebrand, abfackeln, abgefackelt, niedergebrannt, verbrannt, brandbeschleuniger, brandstiftung, brandstifter, anzünden, angezündet, entzündet, großbrand, flächenbrand, pyromanie, brenzlig, benzin, grossfeuer, pickel, einäschern, feuersbrunst, küchenbrand, anstecken, vernichtung, zerstörung, sonnenbrand, wund, hitze, brennspiritus, rheumatisch, kriegstreiber, löschflugzeug, inflammabilität, feuerspuckerin, schlimm, rapide, platschen, brandanschlag, person, fahrlässig, plötzlich, rot, vermehrung, trommeln, holokaustum, anzünder, peitschen, brandlegung, verqualmen, konflagration, material, grossbrand, feuerspucker, kohleausstieg, atombombenexplosion, wohnhausbrand, abbrennen, scheiterhaufen, holocaust, lichterbaum, gefühl, anmachen, wabern, brühen, buschbrand
\item[Violence] messer, zustechen, einstechen, stechen, zuschlagen, einschlagen, schlagen, töten, ermorden, morden, gewalt, gewaltverbrechen, schleifen, erschlagen, erstechen, schießen, erschießen, packen, beißen, zubeißen, verbeißen, erwürgen, würgen, erdrosseln, zuschnüren, abschnüren, dolch, obstmesser, brechen, zuschnallen, sax, verknoten, abbinden, überschlagen, stich, blockieren, beissen, killen, zubeissen, zubinden, abbeissen, speien, erdrücken, zuzurren, unterschlagen, zuschnappen, totschlagen, serienmord, gewalttat, hals, schäler, niederschlagsmesser, kehle, stachel, abdrücken, verschlagen, abwürgen, meucheln, zustossen, erschiessen, ertränken, liquidieren, festbeissen, hehlen, krampfen, drosseln, stichwaffe, zumachen, sticheln, passieren, garrotte, zuwerfen, schlachten, messerspitze, springmesser, cuttermesser, zusammenknoten, filetiermesser, wälzen, stilett, abschlachten, xylographie, sägemesser, schieben, tötungsdelikt, strangulieren, mörder, geiselnahme, enthaupten, rücken, zuklappen, drossel, vorschlagen, bumsen, durchschlagen, entleiben, mord, abbindung, messerstecherei, verbeissen, aufspielen, zu, schneiden, gefühl, wegbeissen, schnur, reinbeissen
\item[War] krieg, gefecht, kampf, krieger, truppe, truppen, kommandant, kriegsschiff, feind, soldat, offizier, kamerad, stellung, posten, gewehr, maschinengewehr, unteroffizier, general, oberleutnant, leutnant, bunker, graben, schützengraben, panzer, flotte, kriegsflotte, heer, schlachtschiff, bombe, flugzeug, staffel, flieger, kampfflugzeug, kreuzer, zerstörer, flughafen, militärflugzeug, princeps, panzerung, jagdpanzer, häuserkampf, seestreitkraft, hasser, landstreitkräfte, fahnenflucht, partner, löschflugzeug, grenadier, mg, gemeinsam, leichtflugzeug, armada, feuerwerker, flottenkommandant, stadtkommandant, reserveleutnant, milizionär, panzerkampfwagen, bekämpfung, parteifeind, hubschrauberträger, hilfskreuzer, logistikoffizier, geschützturm, zeitsoldat, unterstützung, triere, spähkreuzer, hagelflieger, geisterflotte, höhe, unterseekreuzer, gruppe, luftschutzbunker, geheimdienstoffizier, betonbunker, hauptmann, spielbahn, olt, luftschlag, marine, schädling, vorgefecht, theater, jabo, hubschrauberflotte, flottenstützpunkt, kampfpanzer, luftwaffenleutnant, stabsunteroffizier, schutzstaffel, streubombe, grabenkampf, türstaffel, kampfflieger, pyroklast, harnisch, münze, führer, solarflugzeug, besatzungstruppe, leiter, pulverfass, klüver, treppe, stuka, leutnants, lenkwaffenkreuzer, minensucher, kindersoldat, hindernis, abwehr, kanonenboot, fahrzeug, narkosegewehr, syntagma, büchse, jagdflugzeug, sowjettruppe, fuhrpark, sergeant, rettungsbombe, marinesoldat, kampfpilotin, widersacher, schrotgewehr, flottille, unterfeldwebel, durchmesser, legion, orlogschiff, oberfähnrich, rückzug, solarflieger, weigand, kriegsspiel, jagdflieger, infanterieleutnant, spürpanzer, wachtkommandant, samurai, grünbunker, bomberflotte, schabracke, bau, abwassergraben, düsenjäger, hubschrauberkreuzer, leutnante, unterstand, bootsmann, brigadegeneral, flg, jagdbomber, fairwaybunker, flottenkreuzer, schiessgewehr, landsknechtsoffizier, parade, atombunker, springer, rettungskommandant, kampfschiff, türschwelle, sandbunker, staffeln, presseoffizier, sturzkampfflugzeug, schlachtflotte, wasserlandung, gen, brückenpanzer, fliegerstaffel, artillerieoffizier, landwehroffizier, tornado, front, fusssoldat, feldwebel
\item[Storm] unwetter, donnern, sturm, wolkenbruch, gewitter, orkan, gewittersturm, regnen, donner, prasseln, hagelschauer, hagelschlag, schneesturm, hageln, gewitterregen, donnerwetter, sturmwind, hagelsturm, schneestürme, sturmböen, schneien, schneeregen, regengüssen, regenwetter, regenfall, regengüsse, schneefall, starkregen, gewitterschauer, blitz, regen, wind, windstoß, hagel, windsbraut, niederprasseln, fluchen, schiffen, hineindonnern, niederschlag, fahrwind, schneebö, beschneien, stunde, massregelung, schmuddelwetter, schlossen, platzregen, schneereifen, schlechtwetter, potzblitz, schneiben, caramba, windstoss, fisseln, wetterleuchten, hau, starkregenguss, fahrtwind, einhergehen, dicht, rückenwind, peitschen, brettern, naturgewalt, grollen, regnerisch, pissen, medicane, schnee, gefühlsentladung, heftig, gegenwind, aufhellungsblitz, neuschnee, schneegrenze, flaute, wintereinbruch, hagelkorn, schneegewitter, düsengewitter, sintflut, wucht, graupel, regenblase, zenitalregen, hurrikan, federweisser, hereinschneien, grollend, unpersönlich, husche, verhageln, zurechtweisung, anschneien, reinschneien, hitzegewitter, sturzregen, platschen, starkwind, wettern, regenschauer, sturzflut, bora, verb, bö, trommeln, strafpredigt, umgangssprachlich, bumsen, wassertropfen, hineinschneien, geschosshagel, trinken, tiefschnee, trippeln, omuramba, regenguss, wabern, dunst
\item[Duel] kampf, gegner, duell, klinge, schwert, messer, pistole, zweikampf, feind, sieger, kämpfen, duellieren, waffe, opfer, wunde, stoßen, rammen, wild, erbittert, aufeinander, einschlagen, schlagen, streit, widersacher, gegenüber, obstmesser, messerklinge, verbitterung, energiewaffe, verbittern, niederkämpfen, auf, lenkwaffe, bitterlich, wund, erbfeind, hasser, eines, verwunden, bauernopfer, degenduell, gegenspieler, kurzschwert, hemmungslos, schäler, bajonett, person, niederschlagsmesser, bekämpfung, blatt, streiten, parteifeind, fechten, einhänder, eifern, versus, aufschütten, kopfballduell, knarre, photonentorpedo, gang, wechselseitig, gewinner, stahlklinge, verärgert, messerspitze, springmesser, cuttermesser, bedonnert, stacheldraht, einer, verbittert, revolver, kriegerin, kurzschliessen, diskriminierung, filetiermesser, nebeneinander, ersiegen, bitter, eine, brandopfer, ringen, angriffswaffe, xylographie, sägemesser, mit, kommunikator, zweischneidig, anderen, nach, flamberg, tabakgegner, dienstpistole, gottseibeiuns, antagonist, sichel, gegen, xenophob, kernwaffe, einschneidig, bumsen, gesamtsieger, rittern, komponieren, rennduell, spielsieger, neben, sekundant, klassensieger, pistol, fighten
\item[Overall Danger] einer, kriegsflotte, starkwind, einstechen, geiselnahme, verbrennung, windstoss, kehle, knarre, rückzug, hehlen, streubombe, gewehr, orlogschiff, zubinden, duell, ringen, husche, brandstifter, kernwaffe, reinbeissen, überschlagen, dunst, messer, geheimdienstoffizier, grollend, kampfschiff, feuerspucker, maschinengewehr, kanonenboot, antagonist, hereinschneien, geisterflotte, verbeißen, sowjettruppe, obstmesser, brandstiftung, abbinden, messerstecherei, benzin, gegner, verwunden, lodern, erschießen, leutnante, potzblitz, mit, fuhrpark, spürpanzer, tabakgegner, zu, princeps, sturzregen, zeitsoldat, sturzflut, schneegrenze, erschlagen, wettern, verbrannt, löschen, packen, schlimm, büchse, hagelflieger, stuka, gewitterschauer, fesseln, erwürgen, blockieren, gesamtsieger, fairwaybunker, olt, gefühl, gebäudebrand, hubschrauberflotte, zuschnallen, hageln, waffe, gef, verbrennen, löschflugzeug, feldwebel, beißen, rettungsbombe, wetterleuchten, anmachen, stichwaffe, bomberflotte, münze, regenblase, hubschrauberkreuzer, einhänder, material, totschlagen, schleifen, legion, ersiegen, zuklappen, treppe, kreuzer, garrotte, regenschauer, sturm, kidnapping, luftwaffenleutnant, regenwetter, klassensieger, rettungskommandant, staffeln, landsknechtsoffizier, gewalttat, nach, festbeissen, bedonnert, inflammabilität, kindesentführer, verknoten, tornado, häuserkampf, klüver, pistole, regenguss, unterfeldwebel, hubschrauberträger, einsperren, erschiessen, bitterlich, schützengraben, kidnapper, eines, atombunker, feuerwerker, triere, stechen, geschützturm, beschneien, hitzegewitter, wunde, heftig, widersacher, zumachen, sekundant, angriffswaffe, einschlagen, gegenüber, fahrwind, ertränken, blitz, messerklinge, anstecken, wucht, panzer, unterstützung, photonentorpedo, strangulieren, schlagen, knebeln, verbittern, zuschlagen, pyroklast, stich, höhe, bitter, starkregen, medicane, trippeln, flotte, plötzlich, schnee, schiessgewehr, leichtflugzeug, bau, aufspielen, fisseln, sax, zustechen, prasseln, gewaltverbrechen, fluchen, truppen, niederschlag, jabo, schneefall, rot, offizier, regnerisch, streiten, degenduell, stilett, drosseln, mord, unterstand, holocaust, minensucher, schlechtwetter, lenkwaffenkreuzer, wegbeissen, hauptmann, einhergehen, gegenwind, schneereifen, schrotgewehr, hausbrand, armada, bunker, kommandant, verschlagen, pickel, artillerieoffizier, brandlegung, solarflieger, trinken, milizionär, gottseibeiuns, flächenbrand, leutnants, jagdflieger, wechselseitig, zenitalregen, liquidieren, eifern, explosionsartig, schneiben, verärgert, sticheln, kriegerin, grenadier, schlachtflotte, general, cuttermesser, gefühlsentladung, zurechtweisung, betonbunker, düsenjäger, tötungsdelikt, fighten, weigand, schwert, hals, federweisser, eine, erdrosseln, wohnhausbrand, grossfeuer, hurrikan, brennspiritus, eingesperrt, anderen, sturmwind, gewitter, flugzeug, geiselnehmer, aufeinander, wind, energiewaffe, sintflut, vernichtung, wild, schädling, reserveleutnant, konflagration, gefängnis, vorgefecht, kommunikator, niedergebrannt, sonnenbrand, auf, bauernopfer, leutnant, bö, hau, schäler, brechen, hineindonnern, pulverfass, rückenwind, blatt, gekidnappt, regnen, meucheln, grünbunker, soldat, flamberg, verbittert, fahrlässig, zuwerfen, gewittersturm, person, hemmungslos, gegenspieler, fusssoldat, abbeissen, scheiterhaufen, gefangen, erdrücken, xenophob, kopfballduell, infanterieleutnant, flaute, kriegsschiff, versus, panzerung, fechten, spielbahn, truppe, bekämpfung, gegen, dicht, zubeißen, parteifeind, flugzeugentführer, wolkenbruch, gen, feuersturm, schieben, platzregen, zuschnüren, abbrennen, abschnüren, sieger, spähkreuzer, geschosshagel, naturgewalt, fahnenflucht, rheumatisch, aufschütten, strafpredigt, landstreitkräfte, verhageln, wintereinbruch, niederkämpfen, fahrtwind, krampfen, würgen, gang, aufhellungsblitz, donnern, parade, durchschlagen, jagdbomber, entführen, schneegewitter, passieren, kindersoldat, abbindung, stachel, marine, schlachtschiff, anzünden, schießen, grollen, landwehroffizier, türschwelle, zustossen, verbeissen, besatzungstruppe, schneien, pyromanie, platschen, inhaftieren, bombe, kampfpilotin, einschneidig, leiter, brandopfer, gewalt, dienstpistole, flottille, explosion, gefesselt, zubeissen, schneeregen, brettern, rennduell, wund, filetiermesser, sergeant, enthaupten, panzerkampfwagen, hagelschlag, töten, ermorden, krieg, türstaffel, neuschnee, stellung, niederschlagsmesser, flughafen, klinge, mg, harnisch, schneebö, düsengewitter, wassertropfen, brühen, massregelung, nebeneinander, stacheldraht, speien, luftpirat, kampf, entzündet, lichterbaum, kriegsspiel, zweischneidig, zuschnappen, stahlklinge, gefecht, hagelkorn, kampfflugzeug, atombombenexplosion, bumsen, caramba, revolver, schutzstaffel, theater, omuramba, fahrzeug, peitschen, anzünder, flg, schlachten, wachtkommandant, hasser, springmesser, orkan, unpersönlich, diskriminierung, unteroffizier, schneiden, großbrand, mörder, pissen, schabracke, duellieren, gemeinsam, zuzurren, jagdpanzer, fliegerstaffel, frei, erstechen, donnerwetter, freiheit, morden, narkosegewehr, durchmesser, donner, umgangssprachlich, kidnappen, tiefschnee, springer, posten, kurzschliessen, stoßen, kampfflieger, kriegstreiber, front, hagel, kampfpanzer, hilfskreuzer, regenfall, feind, verqualmen, drossel, syntagma, anschneien, grabenkampf, abwassergraben, erpressen, graupel, dolch, rittern, messerspitze, reinschneien, schmuddelwetter, staffel, kamerad, sturmböen, partner, verb, brandanschlag, marinesoldat, regengüssen, streit, graben, regengüsse, windsbraut, starkregenguss, hitze, brigadegeneral, unwetter, abschlachten, hagelschauer, zerstörer, spielsieger, gefangener, komponieren, angezündet, feuersbrunst, verbitterung, geknebelt, heer, holokaustum, seestreitkraft, bora, feuer, krieger, führer, entleiben, schneesturm, stunde, serienmord, entführer, abgefackelt, rammen, zusammenknoten, bootsmann, gefangenschaft, kurzschwert, oberfähnrich, zerstörung, militärflugzeug, bajonett, hindernis, rapide, käfig, hineinschneien, gewitterregen, vermehrung, xylographie, windstoß, oberleutnant, schiffen, abwehr, festsetzen, wabern, flieger, schanghaien, brenzlig, hagelsturm, niederprasseln, sägemesser, samurai, entführung, schnur, pistol, einäschern, neben, entführt, zweikampf, luftschlag, opfer, küchenbrand, solarflugzeug, unterschlagen, logistikoffizier, wasserlandung, lenkwaffe, abwürgen, kämpfen, rücken, brandbeschleuniger, flottenstützpunkt, flottenkommandant, unterseekreuzer, brennen, sturzkampfflugzeug, killen, presseoffizier, grossbrand, mitgefangener, abdrücken, kohleausstieg, vorschlagen, brand, wälzen, gruppe, schneestürme, sichel, beissen, brückenpanzer, abfackeln, luftschutzbunker, regen, schlossen, gewinner, erbittert, jagdflugzeug, trommeln, buschbrand, flottenkreuzer, stadtkommandant, sandbunker, stabsunteroffizier, feuerspuckerin, erbfeind
\end{description}

==> resources/embedding.tex <==
\begin{description}
\item[Fear] grässlich, Bedrohung, leiden, furchterregend, Angst, erschrocken, Furcht, verschrecken, erbärmlich, hoffnungslos, nervös, lähmen, überwältigen, Schrecken, überwältigend, grauslich, erschrecken, gefahrvoll, verschlimmern, ängstigen, beunruhigend, gefährden, ohnmächtig, entsetzt, wehrlos, Beunruhigung, beunruhigen, schocken, besorgt, unheimlich, scheußlich, schreckhaft, bedrohlich, Panik, verängstigen, verzweifelt, verängstigt, lähmend, unerträglich, schlimm, überwältigt, bedrohen, bedroht, unsäglich, jämmerlich, entsetzlich, beängstigen, fürchterlich, gefährdet, verschüchtern, schrecklich, panisch, höllisch, widerlich, ungeheuerlich, schmerzen, erschreckt, verzweifeln, Schreck, gelähmt, Gefahr, furchtbar, hilflos, gefährlich, verwirren, beunruhigt, erschüttern, schmerzhaft, fürchten, schauerlich, leidend, ängstlich, stottern, zittern, Zittern, schlottern, Gänsehaut, schwitzen, Angstschweiß, Panikattacke
\item[Abduction] entführen, foltern, kidnappen, fliehen, Mordkomplott, aussperren, Gangsterbosses, fesseln, verprügeln, Gewalt, gesperrt, einsperren, geknebelt, entfliehen, verschleppen, kidnappt, eingesperrt, gekidnappt, Entführer, freilassen, gefesselt, flüchten, Kidnapping, knebeln, Gangster, Ganove, entführt, Geisel, Geiselnahme, Gangsterboss, sperren, überfallen, gefangen, Kidnapper, zerren
\item[Fire] zerstören, flammen, Waldbrand, löschen, abgefackelt, verbrennen, Feuer, brennen, verbrannt, Dachstuhlbrand, durchbrennen, explosionsartig, Kaminbrand, Hausbrand, anzünden, Großfeuer, Schwelbrand, Vollbrand, zündeln, niederbrennen, entzündet, zünden, Verbrennung, abbrennen, Brandanschlag, Brandbeschleuniger, Zimmerbrand, niedergebrannt, abgebrannt, Brandstifter, verkohlen, Explosion, Brandausbruch, detonieren, abfackeln, ausbrennen, ausgebrannt, Gebäudebrand, Feuersturm, entzünden, explodieren, Brandnacht, Feuerbrand, Kellerbrand, Wohnungsbrand, angezündet, prasseln, Brandkatastrophe, entflammen, verwüsten, entfachen, Großbrand, Wohnhausbrand, anbrennen, Brandstiftung, lodern, Brand, brennend
\item[Violence] Gewaltverbrechen, umbringen, foltern, erstechen, zerquetschen, schnüren, erwürgen, würgen, abstechen, erschlagen, töten, ermorden, beißen, zustechen, abschnüren, schleifen, morden, Gewalt, verschlingen, zubeißen, zuschnüren, zusammenschlagen, zuschlagen, durchschlagen, durchstechen, schlagen, einschlagen, erdrosseln, Dolch, losschlagen, erschießen, packen, stechen, schießen, einschießen, schlitzen, verbeißen, durchbeißen, Messer, zerbeißen, durchbohren, durchstecken, einstechen, vergewaltigen, Vergewaltigung, röcheln, blutüberströmt, verbluten, bluten, Blut, Blutbad, blutend, blutig, verblutet, entstellt, Stichwunde, Schusswunde, Bisswunde, erstochen, erschossen, erwürgt, erdrosselt, ermordet, gemordet, Mord, Totschlag, Opfer, Menschenopfer, geopfert, opfern, Opferung, Massaker, massakrieren, Amoklauf, Amok, Anschlag, Mordanschlag, Mordkomplott, Ermordung, Waffe, Gewehr, Pistole, Revolver
\item[War] Oberleutnant, Flugzeug, Gefecht, Regimentskommandeur, Kampfschiffe, Stellung, Kriegsflotte, Kriegsmann, Krieg, Leutnant, Panzerfaust, Schlachtkreuzer, Stabsoffizier, Zerstörer, Oberstleutnant, Schlachtschiffe, Krieger, Kampfflugzeug, Unteroffizier, Geschwader, Bombe, Großkampfschiffe, Truppenführer, Kreuzer, Flieger, Offizier, Marineschiffe, Heer, Marineoffizier, Feind, Bunker, Bataillonskommandeur, Kamerad, Flotte, Truppe, Generalstabsoffizier, Kompaniechef, Generalmajor, Panzer, Graben, Regiment, Truppen, Kriegsschiffes, Artillerieoffizier, Schlachtschiff, Kommandeur, Divisionskommandeur, Flugzeugträger, Panzerschiff, Generalleutnants, Kommandant, Feldwebel, Generalleutnant, Kriegsschiff, Brigadekommandeur, Staffel, Kampf, Maschinengewehr, Kriegsschiffen, Soldat, Schützengraben, Schlachtschiffen, Fregatte, Gewehr, Kriegsschiffe, Armee, General, Posten, Granate, Grenadier, Patrone, Munition, Angriff, Rückzug, Rückzugsgefecht, Angriffsformation
\item[Storm] Dauerregen, Sturmwind, regnen, Schneefällen, Regen, Blitz, Schneestürmen, Sturmböen, donnern, Gewittersturm, Hagelsturm, Orkan, Gewitterwolke, Regengüssen, Regengüsse, Sommergewitter, Regenschauer, Hagelschlag, Unwetter, Donner, Schneesturm, Gewitternacht, schneien, Regenfälle, Gewitterwolken, Schneefälle, Regenwolken, Sturzregen, Wolkenbruch, Schneeregen, Regenschauern, Schneefall, Regenfall, Windstoß, hageln, Sturm, Gewitterschaue, Wolkenbrüche, Föhnsturm, Hagelschauer, Platzregen, Gewitterschauer, Donnerwetter, Regenwetter, Gewitterfront, prasseln, Starkregen, Hagel, Schneetreiben, Schneefalls, Schneebruch, Schneeschauern, Schneeschauer, Windböen, Windbruch, Gewitter, Wind, Gewitterregen, Schneestürme, Starkwind, Hurrikan, Tornado, Welle, Sturmwelle, Bö, Böe, Orkanbö, Orkanböe, orkanartig
\item[Duel] Klinge, duellieren, Widerstandskampf, Ringkampf, abschlagen, Duell, bekämpfen, Zweikampf, verbittern, gegenüberstellen, kämpfend, zusammenschlagen, Pistole, rammen, Schwert, zuschlagen, Streit, schlagen, Endkampf, schleudern, Abwehrkampf, Feind, gegenüberstehen, Faustkampf, stoßen, erbittert, Gegenspieler, Waffe, aufstoßen, losschlagen, Wunde, Opfer, Wurfmesser, kämpfen, Widersacher, Verfolger, Kampf, Sieger, wild, Messer, ankämpfen, verzweifeln, gegenübertreten, Gewehr, aufeinander, Kampfmesser, Gegenüber, Gegner, Attacke, Angriff, Verteidigung
\item[Overall Danger] Attacke, Gewalt, einstechen, Totschlag, Brandnacht, Truppenführer, Ringkampf, Faustkampf, Sturmwelle, Kriegsschiffes, verbeißen, Schneefälle, Oberstleutnant, abschlagen, Regenwetter, Regengüssen, verprügeln, Rückzug, Orkanbö, lodern, erschießen, Feuersturm, entfachen, Brandausbruch, zünden, Artillerieoffizier, Wolkenbruch, erschlagen, Grenadier, Widersacher, verbrannt, löschen, verbluten, Marineoffizier, packen, entfliehen, einschießen, Marineschiffe, fesseln, erwürgen, Opferung, kidnappt, Krieger, Soldat, Offizier, detonieren, Schneeregen, Leutnant, hageln, verbrennen, Kamerad, Gegenspieler, Panzerfaust, ankämpfen, beißen, Kriegsschiffen, gegenüberstehen, Windböen, schleifen, erdrosselt, Gegner, verschlingen, Flugzeug, Gewitterwolke, Gebäudebrand, durchstecken, Schneestürmen, Zimmerbrand, abstechen, Donnerwetter, Gangsterboss, einsperren, Gangster, Generalstabsoffizier, stechen, Kampfmesser, Massaker, Bisswunde, Gefecht, Wunde, schnüren, einschlagen, zerren, Starkwind, Kriegsschiffe, Sturzregen, Messer, Orkanböe, Mordkomplott, Wurfmesser, Kriegsschiff, Brandkatastrophe, Kampfschiffe, schlagen, Schützengraben, knebeln, Vollbrand, verbittern, Waldbrand, Kaminbrand, zuschlagen, Truppe, Granate, Großbrand, Dachstuhlbrand, Kidnapping, Opfer, zustechen, prasseln, Gangsterbosses, flammen, Gewitterschauer, Widerstandskampf, Staffel, entstellt, ausbrennen, Abwehrkampf, Explosion, Schneetreiben, Gewitterfront, Panzer, Regenfälle, Schneesturm, Verteidigung, Generalleutnant, orkanartig, schlitzen, Hagelsturm, Dauerregen, Flieger, Verfolger, aufstoßen, niederbrennen, Sturm, Gewitternacht, Zweikampf, Klinge, Amoklauf, explosionsartig, erschossen, Schneeschauer, Wind, Brigadekommandeur, zerbeißen, erdrosseln, Schneebruch, Unteroffizier, Schlachtkreuzer, Starkregen, eingesperrt, Hurrikan, Kompaniechef, aufeinander, Feuer, wild, Wolkenbrüche, Truppen, niedergebrannt, flüchten, Angriff, überfallen, Waffe, Geisel, gekidnappt, regnen, Schusswunde, blutig, Kampfflugzeug, durchbeißen, entflammen, Brandstifter, umbringen, Gewittersturm, Schlachtschiff, gefangen, Hausbrand, Revolver, Schlachtschiffen, gegenübertreten, blutüberströmt, Gewitterwolken, Hagelschlag, Generalleutnants, Flugzeugträger, abgebrannt, Welle, Gewitterschaue, zubeißen, Krieg, Kommandant, zuschnüren, kämpfend, Endkampf, abbrennen, abschnüren, Maschinengewehr, durchbrennen, Bö, Stichwunde, Geschwader, zündeln, würgen, Angriffsformation, donnern, verschleppen, durchschlagen, entführen, Regenfall, Oberleutnant, durchstechen, anzünden, schießen, losschlagen, Streit, schneien, Windbruch, Heer, verwüsten, Kriegsmann, Schlachtschiffe, Schwert, Regenschauern, Föhnsturm, Amok, Kellerbrand, gefesselt, Ermordung, Rückzugsgefecht, Schwelbrand, General, massakrieren, töten, ermorden, Schneefalls, Brandanschlag, Anschlag, Generalmajor, Verbrennung, röcheln, opfern, Windstoß, Gewaltverbrechen, Kreuzer, entzündet, durchbohren, ermordet, Hagelschauer, gesperrt, Blitz, Böe, Sommergewitter, Patrone, Tornado, Brand, Divisionskommandeur, Munition, duellieren, Wohnhausbrand, Gewehr, Kommandeur, bekämpfen, Gewitterregen, blutend, erstechen, morden, Schneefällen, kidnappen, explodieren, Großfeuer, stoßen, Zerstörer, Brandbeschleuniger, aussperren, erstochen, Gewitter, Bombe, ausgebrannt, Pistole, Blut, Mordanschlag, Dolch, erwürgt, Blutbad, freilassen, Graben, angezündet, Feuerbrand, geknebelt, Menschenopfer, Posten, Feldwebel, Wohnungsbrand, Brandstiftung, Panzerschiff, Hagel, fliehen, Fregatte, abgefackelt, rammen, Schneeschauern, Feind, gemordet, verzweifeln, schleudern, Kampf, Bataillonskommandeur, Mord, Kriegsflotte, Duell, Regen, Unwetter, Armee, entführt, Donner, Geiselnahme, zusammenschlagen, Schneefall, gegenüberstellen, brennend, verblutet, zerquetschen, kämpfen, Platzregen, Regengüsse, Sturmböen, zerstören, Vergewaltigung, Regimentskommandeur, Regenwolken, anbrennen, Bunker, brennen, entzünden, Sturmwind, Gegenüber, verkohlen, Orkan, Regenschauer, Entführer, Ganove, Schneestürme, Stabsoffizier, vergewaltigen, abfackeln, foltern, erbittert, Großkampfschiffe, Regiment, sperren, geopfert, Flotte, Kidnapper, Stellung, bluten, Sieger
\end{description}

==> resources/false_positives_fear.tex <==
\begin{tabular}{lrr}
\toprule
{} &  False Positives &  TP Ratio \\
word         &                  &           \\
\midrule
schrecklich  &               15 &      0.50 \\
schlimm      &               13 &      0.24 \\
Gefahr       &                9 &      0.25 \\
furchtbar    &                5 &      0.38 \\
leiden       &                5 &      0.29 \\
Angst        &                4 &      0.83 \\
gefährlich   &                4 &      0.33 \\
unheimlich   &                4 &      0.00 \\
erschrecken  &                3 &      0.50 \\
fürchterlich &                3 &      0.00 \\
\bottomrule
\end{tabular}


==> resources/good_words_fear.tex <==
\begin{tabular}{lrr}
\toprule
{} &  True Positives &  TP Ratio \\
word        &                 &           \\
\midrule
Angst       &              20 &      0.83 \\
schrecklich &              15 &      0.50 \\
zittern     &               9 &      0.90 \\
Furcht      &               6 &      0.86 \\
Zittern     &               5 &      0.71 \\
bedrohen    &               5 &      1.00 \\
schlimm     &               4 &      0.24 \\
Gefahr      &               3 &      0.25 \\
schrecken   &               3 &      0.75 \\
furchtbar   &               3 &      0.38 \\
\bottomrule
\end{tabular}


==> resources/word_ratio_flop.tex <==
\begin{tabular}{lr}
\toprule
{} &  FP Ratio \\
word          &           \\
\midrule
überfallen    &       inf \\
Pistole       &       inf \\
sperren       &       inf \\
prasseln      &       inf \\
regnen        &       inf \\
vergewaltigen &       inf \\
durchbohren   &       inf \\
morden        &       inf \\
Feind         &       inf \\
Gewalt        &       inf \\
Gewitter      &       inf \\
Mord          &       inf \\
löschen       &       inf \\
Prasseln      &       inf \\
blutig        &       inf \\
Stellung      &       inf \\
graben        &       inf \\
flammen       &       inf \\
ermorden      &       inf \\
kämpfen       &       inf \\
\bottomrule
\end{tabular}


==> resources/word_ratio_top.tex <==
\begin{tabular}{lr}
\toprule
{} &  TP Ratio \\
word         &           \\
\midrule
würgen       &       inf \\
donnern      &       inf \\
brennend     &       inf \\
Bö           &       inf \\
rammen       &       inf \\
röcheln      &       inf \\
zuschlagen   &       inf \\
zerren       &       inf \\
Hagel        &       inf \\
Kampf        &       inf \\
Donner       &       inf \\
schießen     &       inf \\
verschlingen &       inf \\
Sieger       &       inf \\
explodieren  &       inf \\
erwürgen     &       inf \\
Sturmwind    &       inf \\
entfliehen   &       inf \\
entstellt    &       inf \\
gefangen     &       inf \\
\bottomrule
\end{tabular}

